The Implications of Tolerance Optimization on Compressor Blade Design

Geometric variability increases performance variability and degrades the mean performance of turbomachinery compressor blades. These detrimental effects can be reduced by using robust optimization to design the blade geometry or by imposing stricter manufacturing tolerances. This paper presents a novel computational framework for optimizing compressor blade manufacturing tolerances, and incorporates this framework into existing robust geometry design frameworks. Optimizations of an exit guide vane geometry are conducted. The single-point optimal geometry is found to depend on the manufacturing tolerances due to a switch in the dominant loss mechanism. Multi-point geometry optimization avoids this switch so that the geometry and tolerance optimization problems are decoupled.

==> sens.tex <==
\section*{SENSITIVITY ANALYSIS}

The sensitivity of the objective function and constraints appearing in (\ref{eq:opt}) with respect to the design variables are needed by the optimizer to determine the search direction on each optimization iteration. In this section, the numerical procedure for computing the required sensitivities is described.

\subsection*{Pathwise Sensitivity Method}

The pathwise sensitivity method is used to compute the sensitivity of the mean quantities of interest to the design variables. The pathwise approach is well suited to computing these sensitivities since the pathwise derivative can be readily computed from the K-L expansion. The pathwise sensitivity method relies upon interchanging the differentiation and expectation operators. For example, the sensitivity of the mean loss coefficient with respect to a nominal design variable $d_j$ can be computed as

\begin{equation}
\frac{\partial}{\partial d_j}\mathbb{E}[\loss(\samp)] = \mathbb{E}\left[\frac{\partial}{\partial d_j}\loss(\samp)\right].
\end{equation}
The sensitivity $\partial \loss(\samp)/\partial d_j$ represents the sensitivity of the loss coefficient with respect to changing the design variable $d_j$ for a fixed ``path'', i.e. for a fixed realization of the i.i.d Gaussian random variables $\xi_i(\samp)$ in the K-L expansion (\ref{eq:kl}). Replacing the expectation with its Monte Carlo sample average estimate gives

\begin{equation}
\frac{\partial \overline{\loss}}{\partial d_j} = \frac{1}{N_{MC}}\sum_{n=1}^{N_{MC}}\frac{\partial \loss_n}{\partial d_j}.
\end{equation}
The sensitivity of the mean loss coefficient with respect to the tolerance variables is computed similarly:
\begin{equation}
\frac{\partial \overline{\loss}}{\partial \sigma_j} = \frac{1}{N_{MC}}\sum_{n=1}^{N_{MC}}\frac{\partial \loss_n}{\partial \sigma_j}.
\end{equation}

\subsection*{Sample Path Sensitivity}

Computing the sensitivity of the outputs of interest with respect to the tolerance design variables requires an additional step. By the chain rule, the sensitivity can be expanded as
\begin{equation}
\frac{\partial \loss_n}{\partial \sigma_j} = \frac{\partial \loss_n}{\partial e_n}\frac{\partial e_n}{\partial \sigma_j}.
\end{equation}
The first term represents the sensitivity of the output of interest with respect to perturbing the error field. The second term represents the sensitivity of a particular realization of the random field $e(s)$ to a perturbation in one of the tolerance design variables $\sigma_j$. 

TODO: complete

\begin{equation}
e(s,\samp) = \sigma(s)\tilde{e}(s,\samp),
\label{eq:corr}
\end{equation}
We assume that it is impossible to achieve zero variance anywhere on the blade surface. Thus, the standard deviation is constrained to be positive everywhere, since if $\sigma(s)$ goes to zero at some location $s_0$, this implies that there is no geometric variability at $s_0$. 

\subsection*{Shape Sensitivities}

The shape sensitivities $\partial \loss_n/\partial d_j$ and $\partial \loss_n/\partial e_n$ are computed using a second order finite difference approximation. The sensitivities are estimated by introducing a small perturbation $\delta$ to each design variable individually, and computing the resulting change in the quantities of interest.
% COMMENTED
%The sensitivity of the loss coefficient to the nominal design variable $d_j$ can be estimated as
%
%\begin{equation}
%\frac{\partial \loss_n}{\partial d_j} \approx \frac{\loss_n(d_j + \delta) - \loss_n(d_j - \delta)}{2\delta}
%\end{equation}
% COMMENTED
Although this requires a flow solution to be recomputed for each design variable, this computational cost is relatively low since only a small number of iterations are required to reconverge the flow solution at the perturbed state.

==> tol_opt.tex <==
\section{Tolerance Design Framework}

In this section, we present a framework for designing the manufacturing tolerances of compressor blades. We frame tolerance design as an optimization problem which is solved using a gradient-based technique. 

\subsection{Manufacturing Tolerance Model}

The precision of a manufacturing process can be specified in terms of its spread, defined as some multiple of the standard deviation of the dimension of interest, where a dimension refers to the size of a particular feature \cite{kane_1986}. To specify manufacturing tolerances around a compressor blade surface, we specify the process spread, equal to the standard deviation $\sigma(s)$, at every point on the blade surface. The relation between tolerances and variance is illustrated in figure~\ref{fig:tol_var}. The leading edge of the nominal blade geometry is shown in black. The $2\sigma(s)$ bounds on the geometric variability are shown in dashed red lines, and sample realizations of manufactured blade geometries are plotted in color. The left figure demonstrates loose tolerances, where larger variations are allowed as compared to the case where strict tolerances are imposed, shown on the right. The variance is also non-stationary, decreasing near the leading edge in both cases.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.45\textwidth]{figs/loose_tol}
\includegraphics[width=0.45\textwidth]{figs/strict_tol}
\end{center}
\caption{Illustration of loose (left) and strict (right) tolerances near the leading edge of a compressor blade}
\label{fig:tol_var} 
\end{figure*}

The standard deviation field $\sigma(s)$ is represented using a cubic B-spline basis:
\begin{equation}
\sigma(s) = \sum_{i = 1}^{N_\sigma}\sigma_i B_{i}(s),
\end{equation}
where the $B_{i}(s)$ are cubic B-spline basis functions. This choice of basis ensures that the manufactured blade surfaces have continuous curvature, i.e. have no sharp edges. The manufacturing tolerances are parameterized by the vector $\tol = \{\sigma_i\}_{i=1}^{N_\sigma}$.

\subsection{Optimization Framework}

In the proposed tolerance optimization framework, the mean compressor performance is controlled by specifying $\sigma(s)$. We focus on optimizing the mean performance, as opposed to other statistics such as the variance, since evidence from previous robust optimizations of compressor blades found that optimizing the mean performance tends to also reduce the performance variability relative to the baseline design \cite{bestle_2010, garzon_thesis}.  

Since the mean shift in loss coefficient is sensitive to the flow incidence, we design the manufacturing tolerances to minimize the mean loss coefficient over a range of incidence angles by adopting a multi-point design strategy similar to that used in \cite{bock_2002} and \cite{koller_2000}. A set of $N_p$ design points is chosen, each corresponding to an incidence angle. A weighted objective function is defined as the weighted sum of the loss coefficient at each incidence angle, i.e.
\begin{equation}
J := \sum_{i=1}^{N_p} w_i \loss(\beta_i),
\end{equation}
where the weight vector $\mathbf{w} = \{w_1,...,w_{N_p}\}$ weights the relative importance of different incidence angles. The weight vector is chosen so that the multi-point objective function $J$ approximates a weighted integral of the loss coefficient:
\begin{equation}
\sum_{i=1}^{N_p} w_i \loss(\beta_i) \approx \int_\mathcal{B} W(\beta) \loss(\beta)\, d\beta,
\end{equation}
where $W(\beta)$ is a weighting function and $\mathcal{B} = [\beta_1^l,\beta_1^u]$ is the incidence range of interest. Choosing $N_p = 3$ equispaced points and a loss weight vector $\mathbf{w} = \{1/4, 1/2, 1/4\}$ approximates the average loss computed using a trapezoidal integration rule.

The tolerance design process determines where on the blade surface the tolerances should be reduced to have the most benefit, i.e. to provide the greatest reduction in the mean loss coefficient. This is achieved by constraining the level of manufacturing variability, and minimizing the weighted mean loss $\E[J]$. To quantify the level of variability, we introduce the function $V(\tol)$, equal to the integral of the standard deviation of the random field that models the manufacturing variations over the blade surface:
\begin{equation}
V(\tol) = \int_S \sigma(s;\tol)\, ds.
\label{eq:variability}
\end{equation}
Reducing $V$ implies stricter tolerances and therefore increased manufacturing cost. In the optimization, the standard deviation is also bounded from above by a specified value $\sigma_{max}$ to ensure that the optimizer does not trade increases in the variability in regions of low mean loss sensitivity for decreases in high sensitivity regions and drive $\sigma(s)$ to zero. The optimization problem for designing the tolerances is summarized below:
\begin{equation}
\begin{aligned}
& \tol^* =
& & \underset{\tol}{\arg \min}
& & \E[J(\samp,\tol)] \\
& & & \ \ \ \ \text{s.t.}
& & V(\tol) = V_b \\
& & & & & 0 \leq \sigma(s) \leq \sigma_{max}.
\end{aligned}
\label{eq:tol_opt}
\end{equation}

The sample average approximation (SAA) method, also referred to as sample path optimization, is used to compute an approximate solution of (\ref{eq:tol_opt}). The SAA method replaces the objective function $\E[J(\samp,\tol)]$ with a Monte Carlo estimate $\hat{\mu}_J^{(N)}(\tol)$ computed using a fixed set of random inputs, i.e. a fixed set of realizations $\{\bxi^{(n)}\}_{n=1}^{N}$ of the random input vector used to generate realizations of the error field $e(s,\samp)$. Fixing the random inputs transforms the stochastic optimization problem (\ref{eq:tol_opt}) into a deterministic optimization problem. The solution of the deterministic optimization problem, denoted $\hat{\tol}^*_N$, is an estimator of the true solution $\tol^*$. To solve the deterministic optimization problem that approximates the stochastic problem (\ref{eq:tol_opt}), the sequential quadratic programming (SQP) method is used. SQP is a gradient-based method for solving nonlinear constrained optimization problems. More details on SQP can be found in reference \cite{powell_1978}.

The gradient of $\hat{\mu}_J^{(N)}$ with respect to the tolerance design variable $\sigma_i$ is computed by interchanging differentiation and summation:
\begin{equation}
\frac{\partial \hat{\mu}_J^{(N)}}{\partial \sigma_i} = \frac{1}{N}\sum_{n=1}^{N}\frac{\partial J_n}{\partial \sigma_i}.
\end{equation}
Since we are using the SAA method, the derivatives $\partial J_n/\partial \sigma_i$ represent the sensitivity of the random functional $J(\samp,\tol)$ for a particular realization of the random field $e_n \equiv e(s,\bxi^{(n)})$ where all random inputs are held fixed. The sensitivity $\partial J_n/\partial \tol$ is computed using the chain rule:
\begin{equation}
\frac{\partial J_n}{\partial \sigma_i} = \frac{\delta J_n}{\delta e_n}\frac{\partial e_n}{\partial \sigma_i}, \ \ \ \ i = 1,...,N_\sigma
\end{equation}

To compute the sample path sensitivity $\partial e_n/\partial \sigma_i$, we first define the random field $\tilde{e}(s,\samp) = e(s,\samp)/\sigma(s)$. The random field $\tilde{e}(s,\samp)$ has the same correlation function as $e(s,\samp)$, and the variance of $\tilde{e}(s,\samp)$ is equal to one everywhere. Realizations of the random field $e(s,\samp)$, which has variance $\sigma^2(s)$, can be produced by simulating the unit variance random field $\tilde{e}(s,\samp)$ and scaling the realizations by $\sigma(s)$. The sample path sensitivity of a realization $e_n(s)$ with respect to the tolerance design variable $\sigma_i$ is computed using the chain rule:
\begin{equation}
\frac{\partial e_n(s)}{\partial \sigma_i} = \frac{\partial e_n(s)}{\partial \sigma(s)}\frac{\partial \sigma(s)}{\partial \sigma_i} = \tilde{e}_n(s) B_{i}(s),
\end{equation}
where $B_{i,n}(s)$ is the $i^\text{th}$ B-spline basis function used to represent $\sigma(s)$.

\subsection{Application}

We first optimize the manufacturing tolerances for the UTRC exit guide vane. We use $N_p = 3$ design points at $\beta_1 = 38.7^\circ$, $43.2^\circ$, and $47.7^\circ$ and a loss weight vector $\mathbf{w} = \{1/4,\ 1/2,\ 1/4\}$. The total variability, as quantified by Equation (\ref{eq:variability}), is constrained to be 98\% of the baseline total variability, and the standard deviation is constrained to be below the baseline value of $\sigma/c = 8.0 \times 10^{-4}$ at all points on the blade surface. The standard deviation is represented using $N_\sigma = 41$  basis functions, and the knot spacing is reduced near the leading edge, since previous studies of the impact of geometric variability on compressor performance suggest that most of the increase in loss results from imperfections near the leading edge \cite{garzon_2003}. The optimal tolerance scheme is potted in Figure \ref{fig:uti_tol_sigma}. We only show the leading edge since the optimal standard deviation is equal to the baseline value of $8.0 \times 10^{-4}$ everywhere outside of this region.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.5\textwidth]{figs/tol_opt_min_mean_loss_var_const_base_uti}
\caption{Optimal standard deviation $\sigma(s)/c$ for the UTRC blade. The lower surface is the pressure side, and the upper surface is the suction side.}
\label{fig:uti_tol_sigma}
\end{figure}

The optimal tolerance scheme follows a ``double bow-tie'' pattern: the level of variability is reduced on either side of the leading edge, with the greatest reduction on the pressure side of the blade. The optimal tolerances reduce the extent of flow separation for the manufactured blades at both high and low incidence, which reduces the mean loss as illustrated in Figure \ref{fig:uti_tol_opt_loss_bucket}. For the range of incidence angles considered, the average reduction in the mean shift in the loss coefficient achieved by optimizing the tolerances was 49\%.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.5\textwidth]{figs/loss_bucket_multi_point_M_0p73_min_mean_loss_var_const_base_uti}
\caption{Loss coefficient versus incidence angle for the UTRC exit guide vane}
\label{fig:uti_tol_opt_loss_bucket}
\end{figure}
